Physical Design using Differentiable Learned Simulators

Designing physical artifacts that serve a purpose - such as tools and other functional structures - is central to engineering as well as everyday human behavior. Though automating design has tremendous promise, general-purpose methods do not yet exist. Here we explore a simple, fast, and robust approach to inverse design which combines learned forward simulators based on graph neural networks with gradient-based design optimization. Our approach solves high-dimensional problems with complex physical dynamics, including designing surfaces and tools to manipulate fluid flows and optimizing the shape of an airfoil to minimize drag. This framework produces high-quality designs by propagating gradients through trajectories of hundreds of steps, even when using models that were pre-trained for single-step predictions on data substantially different from the design tasks. In our fluid manipulation tasks, the resulting designs outperformed those found by sampling-based optimization techniques. In airfoil design, they matched the quality of those obtained with a specialized solver. Our results suggest that despite some remaining challenges, machine learning-based simulators are maturing to the point where they can support general-purpose design optimization across a variety of domains.

==> Inverse Design/math_config.tex <==
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\E}{\mathop{\mathbb{E}}}


\newcommand{\udist} [1]{\ensuremath{\mathcal{U}({#1})}}

\definecolor{zgray}{RGB}{0,187,214} % sim obs
\definecolor{zgray}{RGB}{225,0,124} % pink
\definecolor{zgray}{RGB}{239,164,0} % yellow
\definecolor{zgray}{RGB}{34,139,34} % green
\definecolor{zgray}{RGB}{70,70,70} % gray

% \definecolor{zcyan}{RGB}{0,187,214} % sim obs
% \definecolor{zpink}{RGB}{225,0,124} % pink
% \definecolor{zyellow}{RGB}{239,164,0} % yellow
\definecolor{zgreen}{RGB}{34,139,34} % green
% \definecolor{zgray}{RGB}{70,70,70} % gray

%% ================== GENERAL ======================= %%
\newcommand{\Identity}{{I}}
\newcommand\norm[2]{\left\lVert#1\right\rVert_{#2}}
\newcommand{\hdg}[1] {\noindent \textbf{#1} }

%% ================== OBSERVATIONS ================== %%
\newcommand{\real}{{real}}
\newcommand{\simu}{{sim}}

\newcommand{\muk}  {{\ensuremath{ {\boldsymbol{\mu}_k} }}}
\newcommand{\Sigmak}  {{\ensuremath{ {\boldsymbol{\Sigma}_k} }}}
\newcommand{\mub}  {{\ensuremath{ {\boldsymbol{\mu}} }}}
\newcommand{\Sigmab}  {{\ensuremath{ {\boldsymbol{\Sigma}} }}}


\newcommand{\distsymb}  {{\ensuremath{ {p} }}}

% \newcommand{\tool}  {{\ensuremath{ {\boldsymbol{\tau}} }}}
% \newcommand{\Tools}  {{\ensuremath{ {\mathcal{T}} }}}
% \newcommand{\ctx}  {{\ensuremath{ {\boldsymbol{\kappa}} }}}
% \newcommand{\Ctxs}  {{\ensuremath{ {\mathcal{K} }}}}

% Updated with Pete's Notation
\newcommand{\ctx}  {{\ensuremath{ {\boldsymbol{c}} }}}
\newcommand{\Ctxs}  {{\ensuremath{ {\mathcal{C} }}}}
\newcommand{\tool}  {{\ensuremath{ {\boldsymbol{d}} }}}
\newcommand{\Tools}  {{\ensuremath{ {\mathcal{D}} }}}

%% ================== PARAMETERS ================== %%
\newcommand{\param}  {{\ensuremath{ {\boldsymbol{\xi}} }}}
\newcommand{\paramscalar}  {{\ensuremath{\xi} }}
\newcommand{\paramdistpar}  {\ensuremath{ {\boldsymbol{\phi}} }}
\newcommand{\paramdist}  {\ensuremath{ q_\paramdistpar }}
\newcommand{\prior}[2]  {\ensuremath{ \distsymb^{#1}(#2) }}
\newcommand{\paramprior}[1]  {\ensuremath{ \distsymb^{#1}(\param) }}

\newcommand{\paramdistr}  {\paramdistC(\param|\reward)}
\newcommand{\paramsimr}  {\param~\sim~\paramdistr}
\newcommand{\paramdistq}  {\paramdistC(\param)}
\newcommand{\paramsim}  {\param~\sim~\paramdistq}
\newcommand{\gradparam}  {\ensuremath{\boldsymbol{\nabla_\param} }}
\newcommand{\paramsample}  {{\ensuremath{ \param \sim \paramdist }}}

% other params
\newcommand{\realparam}  {\param_{\real}}
\newcommand{\realparamdistpar}  {\ensuremath{ {\boldsymbol{\gamma}} }}
\newcommand{\latentparam}  {\ensuremath{ {\boldsymbol{z}} }}
%colored
\newcommand{\paramdistparC}  {\textcolor{zyellow}{\paramdistpar}}
\newcommand{\latentparamC}  {\textcolor{zgreen}{\latentparam}}
\newcommand{\paramdistC}  {\ensuremath{ q_{\paramdistparC} }}
%\newcommand{\paramdistlatentC}  {\ensuremath{ q_{\paramdistparC|\latentparamC} }}

\newcommand{\paramdistappC}  {\ensuremath{ \widetilde{q}_{\paramdistparC} }}
%\newcommand{\realparamdistparC}  {\textcolor{zgray}{\realparamdistpar}}


\newcommand{\Y}  {\ensuremath{ \boldsymbol{y} }}
\newcommand{\Yt} {\ensuremath{y(t)}}
\newcommand{\Ytp} [1]{\ensuremath{\tilde{y}_{#1}(t)}}

\newcommand{\dyn} {\ensuremath{f}}

\newcommand{\traj} {\ensuremath{\tau}}
\newcommand{\Tp} [1]{\ensuremath{\traj_{#1}}}
\newcommand{\Tpj} [2]{\ensuremath{\Tp{#2}^{#1}}}
\newcommand{\Tsim} {\ensuremath{ \Tp{\param} }}
\newcommand{\Treal} {\ensuremath{ \Tp{\realparam} }}
\newcommand{\statspar}  {\ensuremath{ {\boldsymbol{\zeta}} }}
\newcommand{\statsparC}  {\textcolor{zcyan}\statspar}

\newcommand{\state}  {\ensuremath{ \boldsymbol{x} }}
\newcommand{\stateo}  {\ensuremath{ \boldsymbol{\state_0} }}
\newcommand{\statet} {\ensuremath{ \boldsymbol{\state}_t  }}
\newcommand{\statett} {\ensuremath{ \boldsymbol{\state}_{t+1}  }}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Prob}[2] {\distsymb_{#1}(#2)} %\mathbb{P}
\newcommand{\Probb}[1] {\distsymb_{#1}} %(\cdot)}
\newcommand{\MDP}[1] {\ensuremath{\mathcal{M}^{#1}}}
\newcommand{\StateS}  {\ensuremath{ \mathcal{S} }}
\newcommand{\ActionS}  {\ensuremath{ \mathcal{A} }}
\newcommand{\Param}  {\ensuremath{ \Xi }}
\newcommand{\RewardS} {R}
%\newcommand{\TransitionSym}{\ensuremath{ \Probb{\statett} }} %T_{\param} }}
%\newcommand{\Transition}[1]  {\ensuremath{ \TransitionSym(#1; \param) }}
\newcommand{\statettdist}  {\ensuremath{ \distsymb(\statett|\statet, \policydista; \param) }}
\newcommand{\statettdista}  {\ensuremath{ \distsymb(\statett|\statet; \param) }}
\newcommand{\statettsima}  {\ensuremath{ \statett~\sim~\statettdista }}
\newcommand{\statettsim}  {\ensuremath{ \statett~\sim~\statettdist }}
\newcommand{\InitialSDist}  {\ensuremath{ \distsymb(\stateo) }}
\newcommand{\stateodist}  {\ensuremath{ \distsymb(\stateo) }}
\newcommand{\stateodistr}  {\paramdistC(\stateo|\reward)}
\newcommand{\stateosimr}  {\stateo~\sim~\stateodistr}
\newcommand{\stateosim}  {\ensuremath{ \stateo~\sim~\stateodist }}
% \newcommand{\stateoparamdist}[1]  {\ensuremath{ \prior{#1}{\stateo, \param} }}
\newcommand{\beliefdist} {\ensuremath{ \beta(\stateoparam) }}
\newcommand{\stateoparam} {\ensuremath{\stateo, \, \param}}
\newcommand{\stateoparamdist} {\ensuremath{ p(\stateoparam) }}
\newcommand{\stateoparamsim}[1]  {\ensuremath{ \stateoparam~\sim~\stateoparamdist{#1} }}

% =================== TASKS =================== %
\newcommand{\iterid} {\ensuremath{k}}
\newcommand{\batchid} {\ensuremath{b}}
\newcommand{\taskid} {\ensuremath{i}}
\newcommand{\task} [1]{\ensuremath{\nu_{#1}}}
\newcommand{\numtasks} {\ensuremath{N}}

\newcommand{\iter} {\ensuremath{k}}
\newcommand{\niters} {\ensuremath{N}}
\newcommand{\iterlims} {\ensuremath{\iter=1:\niters}}
\newcommand{\rollout} {\ensuremath{b}}
\newcommand{\nrollouts} {\ensuremath{B}}
\newcommand{\rolloutlims} {\ensuremath{\rollout=1:\nrollouts}}
\newcommand{\dset} {\ensuremath{\mathcal{D}}}
\newcommand{\dseti}[1] {\ensuremath{ \dset^{(#1)}  }}


%% ================== POLICY ================== %%
\newcommand{\policypar}  {{\ensuremath{ {\boldsymbol{\theta}} }}}
\newcommand{\policyparC}  {\textcolor{black}{\policypar}}


\newcommand{\policy} {\ensuremath{\pi}}
\newcommand{\policydista} {\policy_{\policyparC}(\actiont|\statet)}

\newcommand{\Policy} [1] {\ensuremath{\policy_{\policypar}({#1})}}
%\newcommand{\PolicyO}[1] {\ensuremath{\policy_{\policyparopt}({#1})}}
\newcommand{\policydist}  { \policy_{\policyparC} }

\newcommand{\trajdistC}[1]  { \Tp{}~\sim~{ \policydist({#1}) } }
\newcommand{\trajdist}  { p(\Tp{} | \stateoparam) }
\newcommand{\trajdistF}[1]  { p(#1({\Tp{}}) | \stateoparam, \policyparC) }
\newcommand{\trajsim}  { \Tp{}~\sim~\trajdist }

\newcommand{\action}  {\ensuremath{ \boldsymbol{a} }}
\newcommand{\actiont} {\ensuremath{ \action{_t} }}
\newcommand{\actionsim}  {\ensuremath{ \actiont~\sim~\policydista }}

\newcommand{\actionopt} {\ensuremath{ \action^{*} }}
\newcommand{\actioni} {\ensuremath{ \action^{(i)} }}
\newcommand{\paramopt} {\ensuremath{ \param^{*} }}
\newcommand{\parami} {\ensuremath{ \param^{(i)} }}
\newcommand{\cost} {\ensuremath{\reward}}
\newcommand{\costi} {\cost^{(i)}}

% stirring
\newcommand{\ActionSTN}[1]  {\ensuremath{ \mathcal{A}_{#1} }}
\newcommand{\actionTN}[1]   {\ensuremath{ \action_{#1} }}

\newcommand{\As} {\ensuremath{\ActionSTN{cs}}}
\newcommand{\Ap} {\ensuremath{\ActionSTN{dp}}}
\newcommand{\as} {\ensuremath{\actionTN{cs} }}
\newcommand{\ap} {\ensuremath{\actionTN{dp}}}
\newcommand{\apopt} {\ensuremath{\ap^*}}
\newcommand{\Z} {\reward}

\newcommand{\noise}  {\ensuremath{ \epsilon }}
\newcommand{\Ln}  {\ensuremath{\hat{L}^N(\param)}}
\newcommand{\paramjk} [2]{\ensuremath{\param_{#2}^{(#1)}}}


%% ================== COSTS ================== %%
\newcommand{\Ds} {\ensuremath{\Delta}}
\newcommand{\Dsj} [1]{\ensuremath{\Delta_{#1}}}
\newcommand{\Dsjk} [2]{\Dsj{#2}^{#1}}


\newcommand{\DefInt} [4] {\ensuremath{\int\limits_{#1}^{#2} #3\; \mathrm{d}{#4}}}
\newcommand{\Discrep} [2] {\ensuremath{D \big( #1, #2 \big) }}
\newcommand{\Cost} {\ensuremath{\RewardS}}
\newcommand{\CostF} [2] {\ensuremath{\Cost^{#1}(#2)}}
\newcommand{\Reward} [1] {\ensuremath{R(#1)}}
\newcommand{\reward} {\textcolor{zgreen}{\ensuremath{r}}}
\newcommand{\rewardhigh} {\ensuremath{\reward_{high}}}
\newcommand{\rewarddist} {\ensuremath{p(r|\stateoparam, \policyparC)}}
\newcommand{\rewardsim} {\ensuremath{\reward~\sim~\rewarddist}}
\newcommand{\Stats} [1] {\ensuremath{\Phi(#1)}} %\mathlarger

%% ================= Symbols ================= %%
\newcommand\tuple[2]{\ensuremath{\left(#1, #2\right)}}


==> Inverse Design/sections/abstract.tex <==
Designing physical artifacts that serve a purpose---such as tools and other functional structures---is central to engineering as well as everyday human behavior.
Though automating design has tremendous promise, general-purpose methods do not yet exist.
Here we explore a simple, fast, and robust approach to inverse design which combines learned forward simulators based on graph neural networks with gradient-based design optimization.
Our approach solves high-dimensional problems with complex physical dynamics, including designing surfaces and tools to manipulate fluid flows and optimizing the shape of an airfoil to minimize drag.
This framework produces high-quality designs by propagating gradients through trajectories of hundreds of steps, even when using models that were pre-trained for single-step predictions on data substantially different from the design tasks.
In our fluid manipulation tasks, the resulting designs outperformed those found by sampling-based optimization techniques.
In airfoil design, they matched the quality of those obtained with a specialized solver.
Our results suggest that despite some remaining challenges, machine learning-based simulators are maturing to the point where they can support general-purpose design optimization across a variety of domains.

==> Inverse Design/sections/background.tex <==
\section{Background}  % aka Battleground
\label{sec:background} 
Solving inverse problems with physical simulators has a long history in science and engineering, spanning data assimilation for weather modeling \citep{navon2009data}, system identification in robotics \citep{guevara2017adaptable, seita_fabrics_2020}, and tomographic and geophysical imaging \citep{cui2016review, pascual1999review}.
Inverse design can be framed as an inverse problem in which the objective is to optimize design parameters to produce some desired target property.
Simulation-based inverse design has been studied in a variety of disciplines, including nanophotonics \citep{molesky2018inverse}, material science \citep{Dijkstra2021predictive}, mechanical design \cite{coros2013computational}, and aerodynamics \cite{anderson1999aerodynamic, Rhie_1983}.

Classical numerical solvers used for inverse design can be highly accurate, but are often inefficient (making sampling-based inference methods infeasible for high-dimensional designs) and domain-specialized ( prohibiting general-purpose inverse design across domains \citep{choi2021use}). 
Differentiable simulators \citep{freeman2021brax,hu2019difftaichi,Schenck2018SPNetsDF} have recently garnered attention, as they allow for more sample-efficient gradient-based optimization. 
However, like classical solvers, they are still typically narrow in application scope, as many simulation techniques are hard to express as a differentiable program (e.g. constraint dynamics and multiphysics coupling).

The last few years have seen increased interest in using machine learning to accelerate inverse design across a variety of applications \citep[e.g.][]{Challapalli2021inverse,Christensen2020predictive,Bombarelli2018Automatic,Forte2022Inverse,
Hoyer2019neural,Kumar2020Inverse,Li2020efficient,Liu2018Generative,Sha2021Machine,ZHENG2021113894}.
These methods can provide impressive speedups over classical approaches by using learned generative models to propose designs (thus calling an expensive simulator fewer times), or by learning a scoring function which maps designs to target values (replacing the simulator entirely). However, they are based on components with limited out-of-domain generalization,
restricting new designs to configurations near the training data or requiring model refinement.

We instead propose to replace classical simulators with learned simulators.
Like learned scoring functions, learned simulators can be faster than classical simulators \citep{kochkov2021machine,stachenfeld2021learned} and are differentiable when parameterized as a neural network.
Furthermore, learned simulators mimic the underlying physical dynamics independent of the design task and are therefore more likely to generalize.
Physics simulators have been successfully implemented as learned, differentiable models of complex dynamics such as fluids, rigid-body interactions, and soft-body systems \citep{bhatnagar2019prediction,li2020fourier,mrowca2018,Rudy2017data,thuerey2020deep,ummenhofer2020lagrangian,wang2020physicsinformed}. 
Graph-based models in particular are promising candidates for design problems, having demonstrated high accuracy, stability, efficiency, and generalization performance \citep{belbute2020combining, pfaff2021learning,sanchez2020learning}.


However, high-quality forward models do not necessarily translate into better downstream task performance \cite{hamrick2020role,lutter2021learning}. While learned simulators have been used successfully for planning and control in low-dimensional state spaces \citep[up to 21 degrees of freedom (DOF), e.g.][]{bharadhwaj2020model,sanchez2018graph,wang2019benchmarking} or more complex domains with small action spaces \citep[6 DOF, e.g.][]{li2018learning}, 
they require replanning at every timestep to avoid error accumulation. It is not known whether learned simulators can support gradient-based, high-dimensional inverse design which demands high accuracy, well-behaved gradients, long-term rollout stability, and generalization beyond the training data.

Here we study inverse design in non-rigid, graph-based physical systems with up to 625 design dimensions and 2000 state dimensions, over 50--300 timesteps, without replanning after the design period. We show that using gradient-based optimization with learned, general-purpose simulators is an effective choice for inverse design.

==> Inverse Design/sections/design_tasks.tex <==
\section{Design Tasks}
\label{sec:design-tasks}
We formulated a set of design tasks across three different physical domains with high-dimensional state spaces and complex dynamics. Each domain uses a different ground-truth simulator $f_S$, which is used to evaluate designs and pre-train the learned simulator model $f_M$.

\subsection{\twodfluids{}}
\label{sec:2d-fluid-design}

Inspired by existing 2D physical reasoning benchmarks \citep{allen2019tools,bakhtin2019phyre}, these tasks involve creating one or more 2D ``tool'' shapes to direct fluid into a particular goal region (\autoref{fig:2dfluids_results}, \autoref{app:2dfluids}).
We consider three tasks with 4--48 design parameters where the goal is to guide the fluid such that each particle comes as close as possible to the center of a randomly-sampled yellow reward region.
In \contain{}, the joint angles $\phi_\mathrm{joints}$ of a multi-segment tool must be optimized to catch the fluid by creating cup- or spoon-like shapes.
In \ramp{}, the joint angles $\phi_\mathrm{joints}$ of a multi-segment tool must be optimized to guide the fluid to a distant location.
In \maze{}, the rotation $\phi_\mathrm{rot}$ of multiple tools must be optimized to funnel the fluid to the target location.
Fluid dynamics are represented using $10^2$--$10^3$ particles, and unrolled for up to 300 time steps.

The learned model $f_M$ is trained on the 2D WaterRamps dataset released by \citet{sanchez2020learning} which uses the solver in \citet{hu2018moving} to generate trajectories.
The dataset contains scenes with 1--4 straight line segments; no curved lines or large numbers of obstacles are shown.
Therefore, designs which solve \twodfluids{} tasks are necessarily far out of distribution for the learned model.

\subsection{\threedfluids{}}
\label{sec:3d-fluid-design}

To evaluate higher-dimensional inverse design, we created a ``landscaping'' task that requires optimizing a 3D surface to guide fluids into different areas of an environment (\autoref{fig:3dfluids}, \autoref{app:3dfluids}).
Specifically, water flows out of a pipe and onto an obstacle parameterized by $\phi_\mathrm{map}$, a $25 \times 25$ heightmap (625 design parameters).
In \direction{}, $\phi_\mathrm{map}$ is optimized to redirect the fluid stream towards a specified direction.
In \twopools{} and \threepools{}, $\phi_\mathrm{map}$ is optimized to split the fluid stream such that particles hitting the floor land as close as possible to one of two or three specified pools.
Each task has multiple variants, such as different target directions in \direction{}.
The simulation is unrolled for 50 time steps, and contains up to 2048 particles.
The learned model $f_M$ is trained on data generated from the simulator in \citet{bender2015divergence}.

\begin{figure*}[h!]
\centering
\includegraphics[width=0.24\textwidth]{figures/init_airfoil_mesh.png}%
\includegraphics[width=0.24\textwidth]{figures/airfoil_stack.png}%
\includegraphics[width=0.24\textwidth]{figures/airfoil_stats_drag.pdf}%
\includegraphics[width=0.24\textwidth]{figures/airfoil_stats_reward.pdf}
\vspace{-0.25em}
\caption{\airfoil{} results. (a) An initial airfoil design is warped by moving 10 control points (orange dots). The physics model simulates the resulting aerodynamics on a 4158 node mesh, based on which lift and drag are computed. (b) For the task of finding a minimum-drag configuration under constant lift constraint, gradient-based learned design is able to find similar designs to specialized solver \dafoam{}, both using single models and ensembles. (c-d) Larger ensemble sizes of 3--5 achieve a close quantitative match to \dafoam{} for both drag and overall reward.
Shown are means over 10 randomized initial designs, with bootstrapped 95\% confidence intervals.}
\vspace{-0.5em}
\label{fig:airfoil}
\end{figure*}

\subsection{\airfoil{}}
\label{sec:airfoil}

Shape optimization in aerodynamics is one area where gradient-based optimization is routinely applied using traditional simulators \citep{buckley2010airfoil}.
Here, we consider the well-studied task of drag optimization of a 2D airfoil profile (\autoref{fig:airfoil}, \autoref{app:airfoil}).
In this task, a wing is defined using a curve on a 2D mesh, which can be deformed using a set of 10 control points $\phi_\textrm{ctrl}$.
The reward function is formulated as optimizing the wing shape to minimize drag under certain constraints such as constant lift and bounds on the shape to prevent degenerate (e.g. infinitely thin) configurations. 
Lift and drag coefficients are computed by running an aerodynamics simulation on a 4158 node mesh.
The learned model $f_M$ is trained on data generated from the ground-truth simulator $f_S$, for which we use the OpenFOAM solver \cite{openfoam}.

\subsection{Model learning and optimization}

While each domain has a different state space structure and uses a different ground-truth simulator $f_S$, the learned simulators $f_M$ all share the same architecture (with identical hyperparameters in \twodfluids{} and \threedfluids{}, and only minor variations of the hyperparameters for \airfoil{} due to it being a steady state simulation; see \autoref{app:model}). 
The models are trained for next-step prediction on task-independent datasets (random perturbations of the design space for \airfoil{} and \threedfluids{}, and an open-source, qualitatively distinct dataset for \twodfluids{}), and are unrolled for up to 300 time steps during design optimization without further fine-tuning (see \autoref{sec:optimization} for details).



==> Inverse Design/sections/discussion.tex <==
\section{Discussion}

We used state-of-the-art learned, differentiable physics simulators with gradient-based optimization to solve challenging inverse design problems.
Across three domains and seven tasks, which involved designing landscapes and tools to control water flows or optimizing the shape of an airfoil, we demonstrated that gradient descent with pre-trained simulators can discover high-quality designs that match or exceed the quality of those found using alternative methods.
This approach succeeds in a variety of interesting and surprising ways:
it permits gradient backpropagation through complex physical trajectories for hundreds of steps; scales to tasks with large design and state spaces (100s and 1000s of dimensions, respectively); and successfully generates designs which require the learned simulator to generalize far beyond its training data.
In the classic aerodynamics problem of airfoil shape optimization, our approach produces a design comparable to that of a specialized solver using only simple, general-purpose strategies like model ensembling.

While our results have exciting implications for inverse design, they also open up possibilities for explaining everyday human behavior like tool invention---a longstanding puzzle in cognitive science \citep{allen2019tools,osiurak2016,Shumaker2011}. 
With general-purpose learned simulators, we have the potential not just to create highly specialized tools in engineering domains, but also to model everyday tool creation, such as creating a hook from a pipe cleaner, building a blanket fort, or folding a paper boat.

Our approach has limitations that should be visited in future work.
Gradient descent is inappropriate for design spaces with regions of zero gradients, such as in \twodfluids{} tasks where the fluid may not always make contact with the tool (\autoref{fig:mpm_zero_grad}).
Many interesting design tasks also have variably-sized or combinatorial design spaces that cannot easily be optimized with gradient descent, such as computer-aided design (CAD) approaches to 3D modeling.
An exciting future direction will be to integrate general-purpose learned simulators with hybrid optimization techniques such as those used in material science and robotics \citep{chen2020generative,toussaint2018differentiable}.
As learned simulators continue to improve, we could also use them to do even broader cross-domain, multi-physics design.
While challenges remain, our results represent a promising step towards faster and more general-purpose inverse design.

==> Inverse Design/sections/introduction.tex <==
\section{Introduction}
 
Humans are creators.
Our ancestors created stone tools which led to innovations in hunting and food consumption, aqueducts and irrigation systems which revolutionized farming and urban habitation, and more recently, airplanes which let us cross the globe in hours.
Automatically designing objects to exhibit a desired property---often referred to as \emph{inverse design}---promises to transform science and engineering, including aerodynamics \cite{eppler2012airfoil}, material design \cite{butler2016computational}, optics \citep{colburn2021inverse}, and robotics \cite{Gupta2021, xu2021diffsim}.

Despite its promise, widespread practice of inverse design has been limited by the availability of fast, general-purpose simulators.
In science and engineering, many methods rely on specialized ``classical'' solvers, which are handcrafted to simulate a particular physical process.
While accurate and reliable, these solvers can be quite slow, may not provide gradients, and are narrow in their applicability \citep{cranmer2020frontier}.
In robotics and reinforcement learning, simulators are often learned, but accumulate errors over long time horizons and often struggle to generalize beyond their training data \citep{janner2019mbpo,talvitie2014model,venkatraman2015improving}, making them unsuitable for design optimization without further finetuning.

Recently, a class of learned physics simulators based on graph neural networks (GNNs) has been proposed \citep{pfaff2021learning,sanchez2020learning}.
These models have shown success in general-purpose physical prediction, exhibiting high accuracy and generalization ability.
However, this may still be insufficient for inverse design problems, as optimizers can exploit regions in the state space where model predictions are unreliable \citep{lutter2021learning}. Models must therefore be more than just accurate overall: they must also be robust and smooth.
It is unknown whether GNN-based physics simulators exhibit these properties.

\begin{figure*}[!t]
\centering
\includegraphics[width=0.96\textwidth]{figures/design_schematic.pdf}
\vspace{-0.25em}
\caption{Optimizing a physical design. Here, the goal is to direct a stream of water (shown in blue) into two ``pools'' (shown in purple) by designing a ``landscape'' (shown in green) parameterized as a 2D height field. (a) The simulation pipeline takes in a design $\phi$ and initial conditions $\alpha$ and uses the design function $f_D$ to produce an initial state. The simulation is rolled out with a pre-trained learned simulator $f_M$ for $K$ steps, at which point the final state is passed (along with reward parameters $\theta_R$) to the reward function $f_R$, which computes the quality of the design. (b) Each step of optimization involves rolling out the simulation and then adjusting the design ($\phi$) accordingly using an optimizer such as gradient descent or CEM. Shown are selected frames from gradient-based optimization in the \twopools{} task of the \threedfluids{} domain.}
\vspace{-0.5em}
\label{fig:schematic}
\end{figure*}

In this paper, we optimize physical designs by performing gradient descent through pretrained, GNN-based, state-of-the-art learned simulators.
We use this approach to perform successful inverse design without requiring further finetuning of the simulator.
Across two high-dimensional fluid manipulation tasks (\twodfluids{} and \threedfluids{}) and a design task from aerodynamics (\airfoil{}), we show that learned simulators:
(1) produce high-quality designs across diverse physical tasks with complex particle- or mesh-based physics, while using the same underlying GNN architecture;
(2) generalize sufficiently to permit designs far outside their training data;
(3) support gradient-based optimization over hundreds of time steps, through states with thousands of particles, in tasks with up to 625 design parameters (and as a result, produce better designs than sampling-based optimization using a classical simulator); and
(4) can be much faster than specialized simulators used in engineering, while generating designs of similar quality.
Overall, our results are a proof-of-concept for how state-of-the-art learned simulators can be used at scale to optimize designs for different physical tasks.

==> Inverse Design/sections/methods.tex <==
\section{Problem Formulation}

\begin{figure*}[h!]
\centering
\includegraphics[width=0.48\textwidth]{figures/optimization_trajectories_relative.png}%
\hspace{1em}\includegraphics[width=0.16\textwidth]{figures/cem_designs_relative.png}%
\hspace{1em}\includegraphics[width=0.16\textwidth]{figures/happy_glass_barplots_norm_gt_v2.pdf}
\vspace{-0.25em}
\caption{\twodfluids{} results. The state spaces consist of $10^2$--$10^3$ particles and the design spaces of 16--36 parameters. (a) Evolution of designs found by GD-M during optimization for each \twodfluids{} task. Visualizations correspond to simulations of the designs under $f_S$. The design is shown in black, fluid particles in blue, and Gaussian reward in yellow. The transparent particles show the location of fluid for $t<t_K$, and the solid particles show the location of fluid at the final frame $(K=150)$. $r$ denotes reward for the current design.
(b) Final designs found by CEM-M.
(c) Mean reward over 50 reward locations (with bootstrapped $95\%$ confidence intervals) obtained by each optimizer across the \twodfluids{} tasks.  For \contain{} and \ramp{}, results are shown for 16 joints; for \maze{}, results are shown for a $6\times6$ grid of 36 rotors. Across these tasks, GD-M outperforms both CEM-M and CEM-S.}
\vspace{-0.5em}
\label{fig:2dfluids_results}
\end{figure*}

Consider the design task depicted in \autoref{fig:schematic}, in which the goal is to direct a stream of water (shown in blue) into two ``pools'' (shown in purple) by designing a ``landscape'' (shown in green) parameterized as a 2D height field.
Here, an ideal design will create ridges and valleys that direct fluid into the two targets.
In the next sections, we formalize what it means to find and evaluate such a design and discuss our choices for simulator and optimizer.

\subsection{Learned simulators}

To demonstrate the utility of learned simulators for finding physical designs, we rely on the recently developed \mgn{} model \citep{pfaff2021learning}, which is an extension of the GNS model for particle simulation \citep{sanchez2020learning}.
\mgn{} is a type of message-passing graph neural network (GNN) that performs both edge and node updates \citep{battaglia2018relational,gilmer2017neural}, and which was designed specifically for physics simulation.
Here, we briefly summarize how the learned simulator works, and refer interested readers to the original papers for details.

We consider simulations over physical states represented as graphs $G\in\mathcal{G}$.
The state $G = (V, E)$ has nodes $V$ connected by edges $E$, where each node $v\in V$ is associated with a position $\mathbf{u}_v$ and additional dynamical quantities $\mathbf{q}_v$. 
These graphs may be either meshes (as in \mgn{}) or particle systems (as in GNS).
In a mesh-based system (such as \airfoil{}), $V$ and $E$ correspond to vertices and edges in the mesh, respectively.
In a particle system (such as \twodfluids{}), each node corresponds to a particle and edges are computed dynamically based on proximity.
Under this framework, we can also consider hybrid mesh-particle systems (such as \threedfluids{}).
See \autoref{app:model} for model implementation details, and \autoref{app:domains} for details on the representation used for each domain.

The simulation dynamics are given by a ``ground-truth'' simulator $f_S:\mathcal{G}\rightarrow\mathcal{G}$ which maps the state at time $t$ to that at time $t+\Delta t$.
The simulator $f_S$ can be applied iteratively over $K$ time steps to yield a trajectory of states, or a ``rollout,'' which we denote $(G^{t_0}, ..., G^{t_K})$.
Using \mgn{}, we learn an approximation $f_M$ of the ground-truth simulator $f_S$.
The learned simulator $f_M$ can be similarly applied to produce rollouts $(\tilde{G}^{t_0}, \tilde{G}^{t_1},  ..., \tilde{G}^{t_K})$, where $\tilde{G}^{t_0} = G^{t_0}$ represents initial conditions given as input.
We note that a learned simulator allows us to take much larger time-steps than $f_S$, permitting shorter rollout lengths: in our running example, one model step corresponds to 200 internal steps of the classical simulator.
See \autoref{fig:schematic}a for an illustration of simulation using a learned model.

\subsection{Optimizing design parameters}
\label{sec:optimization}

To optimize a physical design, we leverage the pipeline shown in \autoref{fig:schematic}: (1) transform design parameters into an initial scene, (2) simulate the scene using $f_M$ or $f_S$, (3) evaluate how well the simulation achieves the desired behavior, and (4) adjust the design parameters accordingly.

\vspace{-0.5em}
\paragraph{Design parameters}
To produce the initial state $G^{t_0}$, we introduce a differentiable design function $f_D: \Phi\times \mathcal{A} \rightarrow \mathcal{G}$ which maps design parameters $\phi\in\Phi$ and other initial conditions $\alpha\in \mathcal{A}$ to an initial state: $G^{t_0}=f_D(\phi, \alpha)$.
In our landscape design task (\autoref{fig:schematic}), $\phi$ is the 2D height field of the mesh, while $\alpha$ is the non-controllable objects in the scene like the initial position of the fluid.

\vspace{-0.5em}
\paragraph{Maximizing reward}
The reward function $f_R: \mathcal{G}\times\Theta_R\rightarrow\mathbb{R}$ maps the final state of a length-$K$ trajectory ($G^{t_K}$ or $\tilde{G}^{t_K}$) and parameters $\theta_R\in\Theta_R$ to a scalar value.
In our running example, the reward function is defined as the Gaussian likelihood of each fluid particle under the closest ``pool'', averaged across particles (\autoref{fig:schematic}a).

We define the full objective under the ground-truth simulator $f_S$ as $J_S(\phi):=f_R(f_S^{(K)}(f_D(\phi, \alpha)); \theta_R)$, where $f_S^{(K)}$ indicates $K$ applications of the simulator.
We want to find the design parameters that maximize $J_S$, i.e. $\phi^* = \argmax_\phi J_S(\phi)$.
We can approximate this optimization using a learned simulation model instead by maximizing $J_M(\phi):=f_R(f_M^{(K)}(f_D(\phi, \alpha)); \theta_R)$.

\looseness=-1
\paragraph{Optimizers}
Optimal design parameters $\phi^*$ can be found using any generic optimization technique.
Given the differentiability of the learned simulator $f_M$, we are particularly interested in evaluating gradient-based optimization, which requires fewer function evaluations and scales better to large design spaces than sampling-based techniques \citep{bharadhwaj2020model}.
We focus on the Adam optimizer \citep{kingma:adam}, which we use to find $\phi^*$ by computing the gradient $\nabla_\phi J_M(\phi)$.
This involves backpropagating gradients through the reward function $f_R$, length-$K$ rollout produced by $f_M^{(K)}$, and design function $f_D$.

As a baseline, we consider the cross-entropy method (CEM) \citep{rubinstein2004cem}, a gradient-free sampling-based technique that is popular in model-based control \cite{chua2018deep,wang2019benchmarking}.
CEM can be used with any simulator and works by sampling a population of candidates for $\phi$ and evolving them to maximize the reward.
However, CEM requires multiple evaluations of $f_M$ or $f_S$ per optimizer step (depending on the population size, which is 20--40), whereas Adam considers only a single candidate $\phi$ and thus only a single evaluation per step.

Across our design tasks (\autoref{sec:design-tasks}) we compared: gradient descent with the learned simulator (\textbf{GD-M}), CEM with the learned simulator (\textbf{CEM-M}), and CEM with the ground-truth simulator (\textbf{CEM-S}).
In all tasks, $f_S$ is non-differentiable, preventing a comparison to GD-S.
However, in the special case of \airfoil{}, we compare to \textbf{\dafoam{}} \cite{he2020dafoam}, a specialized solver which computes gradients with the adjoint method.

\begin{figure*}[!h]
\centering
\includegraphics[width=0.96\textwidth]{figures/waterworks.pdf}
\vspace{-0.25em}
\caption{\threedfluids{} results found with GD-M or CEM-M and evaluated with $f_S$. Simulations use up to 2000 particles and 625 design parameters. The heightmap of a 2D landscape is optimized to redirect the fluid towards the purple targets; birds eye views of heightmaps  are shown in the upper right corner of each subplot. In this high-dimensional task domain, GD finds designs with high reward (a-c), while CEM fails to find meaningful solutions for \twopools{} (d) as well as the other tasks (\autoref{fig:accuracy_comparison}a).
Each subplot reports the mean reward (r) and bootstrapped [lower, upper] 95\% confidence intervals for the corresponding optimizer and task (averaged over 10 randomized initial designs for each task variation, see \autoref{app:3dfluids}).
}
\vspace{-0.5em}
\label{fig:3dfluids}
\end{figure*}

\looseness=-1
\paragraph{Evaluation}
Unless otherwise noted, we always evaluate the quality of an optimized design $\phi^*$ using the ground-truth objective $J_S(\phi^*)$, regardless of whether $\phi^*$ was found using the learned model $f_M$ (as in CEM-M and GD-M) or the ground-truth simulator $f_S$ (as in CEM-S).
We also use rollouts from $f_S$ to produce visualizations in the figures.


==> Inverse Design/sections/results.tex <==
\section{Results}
\label{sec:results}

Our results show that learned simulators can be used to effectively optimize various designs despite significant domain shift and long rollout lengths.
The same underlying model architecture is used for each domain, highlighting the generality of learned simulators for design. 
Examples of designs found with our approach are available at: \url{https://sites.google.com/view/optimizing-designs}.
Performance is always evaluated using the ground-truth simulator $f_S$ (see \autoref{sec:optimization}).
Here we discuss these results, and compare the capabilities of gradient descent with learned simulators over classical simulators and sampling-based optimization techniques.

\subsection{Overall results}
\label{sec:overall-results}

We first asked whether a learned simulator combined with gradient descent (GD-M) could produce good-quality designs at all.
This approach might fail in various ways: accumulating model error, vanishing or exploding gradients \citep{bengio1994learning}, or domain shift \citep{hamrick2020role}.
However, as the following results show, GD-M produced high-quality designs across all three domains.

\autoref{fig:2dfluids_results}a shows qualitative results for \twodfluids{} (\autoref{sec:2d-fluid-design}), where our approach (GD-M) produces intuitive, functional designs to contain (\contain{}), transport  (\ramp{}), or funnel (\maze{}) the fluid to a target location.
On average, GD-M outperforms CEM-M by 16.1--118.9\%, indicating a substantial benefit of gradient-based optimization.
GD-M also outperforms CEM-S by 3.9--37.5\%, despite using a learned simulator rather than the ground-truth.
However, these design spaces are still relatively small (between 16 and 36 dimensions).
In \threedfluids{} (\autoref{sec:3d-fluid-design}), we substantially increase the dimensionality to a 625-dimensional landscape.
Here, GD-M produces robust designs, creating ridges to re-route water in particular directions or valleys to direct water into pools (\autoref{fig:3dfluids}a-c).
In comparison, CEM-M cannot solve any of these tasks, with performance 30--85$\times$ worse than GD-M.

In \airfoil{} (\autoref{fig:airfoil}b), GD-M recovers the characteristic S-curve shape for a low-drag airfoil under a small angle of attack, and matches the design obtained with \dafoam{}, an adjoint aerodynamics solver which computes close-to-optimal designs for this task.
Specifically, the design obtained with \dafoam{} yields a drag coefficient of 0.01902, while GD-M finds designs with drag between 0.01898--0.01919 depending on ensemble size (see \autoref{sec:ensembles}).
Importantly, \dafoam{}'s solver and optimizer are highly specialized for the particular task of airfoil design, while our approach is more general-purpose in that it requires only trajectory data for training and a generic gradient-based optimizer.

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/episode_joints_ablations_wmaze_norm_v2.pdf}
\vspace{-1.6em}
\caption{
Ablation experiments on the \contain{} and \maze{} tasks. 
(a) Performance of all optimizers increase with rollout length; GD-M performance starts to deteriorate around step 225. (b) In \contain{}, CEM performance drops when increasing the number of joints above 24, while GD-M remains stable. (c) We observe a similar trend with the number of tools in \maze{}. (d) CEM often gets stuck in sub-optimal solutions early in optimization, while GD-M performance continues to increase.}
\vspace{-0.5em}
\label{fig:2dfluids_ablations}
\end{figure*}

\subsection{Model stability \& gradient quality}

We investigated accuracy over long timescales by measuring the effect of rollout length on design quality in \twodfluids{} (\autoref{fig:2dfluids_ablations}a and \ref{fig:hg_episode_sweep_demos}).
Longer rollouts can in principle allow for higher reward in this task as they give the fluid time to settle; however, with learned models, they can also be unstable due to error accumulation \citep{talvitie2014model,venkatraman2015improving}.
Nevertheless, we find that the learned simulator does not seem to be severely impacted by this problem.
Specifically, the quality of designs found by GD-M increases up to 225 steps (\autoref{fig:2dfluids_ablations}a), indicating that the learned simulator's accuracy and gradients remain stable for a surprisingly long time. 
Across the episode lengths evaluated, we find that GD-M outperforms not only CEM-M (by 18.1\% on average) but also CEM-S (by 4.4\% on average).
This indicates that the benefits of a having a learned model that supports better optimization techniques can outweigh the error incurred by long rollouts.

The strong performance of GD-M on longer rollout lengths is noteworthy.
Gradients tend to degrade when passed through chains of many model evaluations, and as a result, previous work generally only optimizes gradients in small action spaces over just a few time-steps \cite{li2018learning}.
We speculate that one reason for the success of GD-M is the addition of noise in training $f_M$, which promotes stability on the forward pass and may also force smoother gradients.


\subsection{Generalization}

Deep networks often struggle to generalize far from their training data \cite{geirhos2018generalisation}.
This poses a problem for design: to produce in-distribution training data, we would already need to know what good designs look like, thus defeating the aim of wanting to find \emph{new} designs.
However, we find that the GNN-based simulators studied here overcome this issue.
As noted in \autoref{sec:2d-fluid-design}, the learned simulator for \twodfluids{} was trained on a pre-existing, highly simplified dataset where only one to four straight line segments interact with a fluid 
(\autoref{app:domains}).
In contrast, the design tasks studied here involve highly articulated, curved obstacles (\contain{}, \ramp{}) or a larger number of obstacles (\maze{}); yet, GD-M still discovers effective designs without requiring any finetuning (\autoref{fig:2dfluids_results}).
We suspect this is because the model is trained to learn local collision rules, making it more robust to global distribution shift.

Using a learned simulator trained in a relatively simple environment has another unexpected advantage.
In rare cases, classical simulators suffer from degenerate behavior around certain edge cases.
For example, with the classical simulator for \twodfluids{}, particles can get stuck in between joint segments, especially when there are a large number of parts or joints (\autoref{fig:mpm_instability}). 
However, since the learned simulator was trained on simpler data where these effects are unobserved, it picks up only on the appropriate collision performance and not the unrealistic edge cases. 
Thus, the learned simulator produces more plausible rollouts than the classical simulator in these cases, and might therefore be a better candidate for producing designs that would transfer to the real world.

\subsection{Improving accuracy with ensembles}
\label{sec:ensembles}

In engineering tasks like \airfoil{}, simulators must be especially accurate, as small differences in the predicted pressure field can cause large errors in lift and drag coefficients.
While GD-M (without ensembling) can produce designs close to \dafoam{}'s, we notice a slightly rounder wing front (\autoref{fig:airfoil}b, bottom) causing a small increase in drag (0.01919 versus 0.01902 in \dafoam{}).

To further improve performance, we implemented an ensemble of 
learned simulators trained on separate splits of the training set.
Ensembles are a popular choice for training transition models for use in control \citep{chua2018deep}, as they can provide higher quality predictions and are more resistant to delusions---a particularly problematic issue for accuracy-sensitive domains such as airfoil design.
During optimization, we make predictions with all models in the ensemble, each trained on a different data split, and average the gradients.
As shown in \autoref{fig:airfoil}b-c, larger ensembles yield designs with significantly lower drag ($\beta = -5.3\times 10^{-5}$, $p = 0.0003$, where $\beta$ is a linear regression coefficient) and higher overall reward ($\beta = 5.6\times 10^{-5}$, $p = 0.0001$), and are able to produce designs very close to the solution found by \dafoam{}, with a drag coefficient of 0.01898 (size-5 ensemble).
Thus, with ensembles, we are able to achieve performant designs with a general-purpose learned simulator, indicating that we can use learned models for design optimization in spaces traditionally reserved for specialized solvers like \dafoam{}.

\subsection{Scalability to larger design spaces}
\label{sec:design-dimensionality}
In larger design spaces, sampling-based optimization procedures quickly become intractable, especially with relatively slow simulators.
We hypothesized that gradient descent with fast, learned simulators could overcome this issue, especially as the size of the design space is increased.
We therefore compared different optimizers on \twodfluids{} as a function of the dimensionality of the design space (the number of tool joints in \contain{} or the number of tools in \maze{}) and on the higher-dimensional \threedfluids{}.

For \contain{} (\autoref{fig:2dfluids_ablations}b), the performance of GD-M increases with the number of joints as increasingly fine grained solutions are made possible.
In contrast, for both CEM-M and CEM-S, design quality deteriorates with more joints as high quality solutions become harder to find with random sampling. In the highest dimensional \contain{} task with 48 tool joints, GD-M outperforms CEM-M by $154.9\%$ and CEM-S by $126.5\%$. 
When CEM does find solutions (\autoref{fig:2dfluids_results}b), they lack global coherence and appear more jagged than solutions found with GD-M.
Similarly, for \maze{} (\autoref{fig:2dfluids_ablations}c), the performance of GD-M is largely unaffected by the number of tools, while the performance of CEM-M and CEM-S both degrade as the design space grows. For the highest dimensional \maze{} problem with 36 joints, GD-M outperforms CEM-M by $207.4\%$ and CEM-S by $133.7\%$.

In the 625-dimensional \threedfluids{} task, CEM-M performs 30--85$\times$ worse than GD-M (\autoref{fig:3dfluids}) despite extensive hyperparameter tuning. This trend held across all tasks (\autoref{fig:accuracy_comparison}a), and even persisted when using fewer control points in the design space (\autoref{fig:design_space_3d}).
This is due not only to \threedfluids{}'s larger design space, but also because this problem requires a globally coherent solution: modifying small areas independently is unlikely to have much effect on the global movement of the fluid.

\subsection{Model speed and sample efficiency}

Learned simulators can provide large speedups over traditional simulators in certain domains by learning to compensate for coarser sub-stepping and making optimal use of hardware acceleration.
In \airfoil{}, although we use a very simple GD setup, our approach is able to find very similar designs as \dafoam{}'s specialized optimizer.
Moreover, our approach requires only 21s (single model) to 62s (size-5 ensemble) on a single A100 GPU, compared to 1021s for \dafoam{} run on an 8-core workstation, despite requiring $10\times$ more optimization steps. 

In \twodfluids{}, the ground-truth simulator runs at a similar speed to the learned model \citep[see][]{sanchez2020learning}, but is non-differentiable and therefore depends on more expensive gradient-free optimization techniques which require more function evaluations.
We use 20--40 function evaluations per optimization step of CEM, compared to a single evaluation with GD (which is about $3\times$ more costly, due to the gradient computation). Thus, GD with a differentiable learned model can be much more efficient than using the ground truth simulator with a sampling-based method.
